Fair Termination of Multiparty Sessions

There exists a broad family of multiparty sessions in which the progress of one session participant is not unconditional, but depends on the choices performed by other participants. These sessions fall outside the scope of currently available session type systems that guarantee progress. In this work we propose the first type system ensuring that well-typed multiparty sessions, including those exhibiting the aforementioned dependencies, fairly terminate. Fair termination is termination under a fairness assumption that disregards those interactions deemed unfair and therefore unrealistic. Fair termination, combined with the usual safety properties ensured within sessions, not only is desirable per se, but it entails progress and enables a compositional form of static analysis such that the well-typed composition of fairly terminating sessions results in a fairly terminating program.

==> transitivity.tex <==

\section{A transitive inference system for fair subtyping}

\begin{table}
  \framebox[\textwidth]{
    \begin{mathpar}
      \inferrule[f-end]{\mathstrut}{
        \End \subt[n] \End
      }
      \and
      \inferrule[f-channel]{
        S \subt[n] T
      }{
        \role\Pol U.S \subt[n] \role\Pol U.T
      }
      % \and
      % \inferrule[f-channel-in]{
      %   U \subt[n_1] V
      %   \\
      %   S \subt[n_2] T
      %   \\
      %   n_1 + n_2 \leq n
      % }{
      %   \role\In U.S \subt[n] \role\In V.T
      % }
      % \and
      % \inferrule[f-channel-out]{
      %   V \subt[n_1] U
      %   \\
      %   S \subt[n_2] T
      %   \\
      %   n_1 + n_2 \leq n
      % }{
      %   \role\Out U.S \subt[n] \role\Out V.T
      % }
      \and
      \inferrule[f-tag-in]{
        \forall i\in I: S_i \subt[n_i] T_i
        \\
        \forall i\in I: n_i \leq n
      }{
        \textstyle
        \Tags\rolep\In\Tag_i.S_i \subt[n] \Tags[i\in I \cup J]\rolep\In\Tag_i.T_i
      }
      \and
      \inferrule[f-tag-out-1]{
        \forall i\in I: S_i \subt[n_i] T_i
        \\
        \forall i\in I: n_i \leq n
      }{
        \textstyle
        \Tags[i\in I]\role\Out\Tag_i.S_i \subt[n] \Tags\role\Out\Tag_i.T_i
      }
      \and
      \inferrule[f-tag-out-2]{
        \forall i\in I: S_i \subt[n_i] T_i
        \\
        \exists i\in I: n_i < n
      }{
        \textstyle
        \Tags[i \in I \cup J]\role\Out\Tag_i.S_i \subt[n] \Tags\role\Out\Tag_i.T_i
      }
    \end{mathpar}
  }
  \caption{\label{tab:subt} Inference system for fair subtyping.}
\end{table}
%
\newcommand{\srel}{\mathcal{S}}
\newcommand{\Sk}{\mathsf{S}} 
%

Given a derivation $D$ of $S\subt[n] T$, we denote by $\Sk(D)$ the set of pairs of sessions types \ple{U,V} such that $U\subt[k]V$ occurs in $D$. 
From the regularity of $S$ and $T$ it follows immediately that $\Sk(D)$ is finite. 

\begin{proposition}
If $D_1$ is a derivation of $S\subt[n_1]T$ and $D_2$  is a derivation of $S\subt[n_2] T$, then 
$\Sk(D_1) = \Sk(D_2)$. 
\end{proposition}
\begin{proof}
We prove $\Sk(D_1)\subseteq\Sk(D_2)$. 
The other inclusion can be proved in the same way. 
Let $\ple{U,V}\in\Sk(D_1)$. 
We reason by induction on the minimum distance $d_{U,V}$ of a judgement $U\subt[k]V$ from the root in $D_1$. 
If $d_{U,V} = 0$, then $U = S$ and $V = T$, then $\ple{U,V}\in\Sk(D_2)$. 
If $d_{U,V} > 0$, then $U\subt[k_1]V$ is the premise of a rule with conclusion 
$\Tags\role\Pol\Tag_i.U_i\subt[h_1]\JTags\role\Pol\Tag_j.V_j$, with $U = U_i$ and $V = V_i$ for some $i \in I\cap J$. 
By induction hypothesis, we have $\ple{\Tags\role\Pol\Tag_i.U_i,\JTags\role\Pol\Tag_j.V_j} \in \Sk(D_2)$, then 
$\Tags\role\Pol\Tag_i.U_i\subt[h_2]\JTags\role\Pol\Tag_j.V_j$ is derived in $D_2$ by a rule where one of the premises is necessarily $U_i\subt[k_2]V_i$ because $i \in I\cap J$. 
Therefore, $\ple{U,V}\in\Sk(D_2)$ as needed. 
\end{proof}

Thanks to the above proposition, we can correctly define 
$\Sk(S,T)$ as $\Sk(D)$ for some derivation $D$ of $S\subt[n] T$. 

\begin{proposition}
If $\ple{U,V}\in\Sk(S,T)$ then $\Sk(U,V)\subseteq\Sk(S,T)$. 
\end{proposition}
\begin{proof}
Since $\ple{U,V}\in\Sk(S,T)$, $S\subt[n]T$ holds by a derivation $D_1$ and $U\subt[k]V$ occurs in $D_1$. 
Hence, it is the root of a subderivatio n $D_2$ of $D_1$ and so 
$\Sk(U,V) = \Sk(D_2) \subseteq\Sk(D_1) = \Sk(S,T)$. 
\end{proof}

\begin{lemma}
  \label{lem:regular_derivation}
  If $S \subt[n] T$, then $S \subt[k] T$ is derivable by a regular proof tree, 
  for some $k \le n$. 
\end{lemma}
\begin{proof}
For all session types $S,T$,  let us define $m_{S,T}\in\N+\set{\infty}$ as follows: 
\[
k_{S,T} \eqdef \min\set{ n \in \N+\set{\infty} \mid S \subt[n] T }
\]
Note that if $S \subt[n] T$ holds, then $m_{S,T}$ is finite and $S\subt[m_{S,T}] T$ holds. 

We prove the thesis by regular coinduction \cite[Prop.~6.1]{Dagnino21}. 
Consider the following set 
\[
\srel \eqdef \set{ U \subt[m_{U,V}] V \mid \ple{U,V}\in \Sk(S,T) }
\]
Clearly, $\srel$ is finite and $S\subt[m_{S,T}] T$ belongs to it and $m_{S,T}\le n$ by definition, hence to conclude we just have to show that every judgement in $\srel$ is the conclusion of a rule in \cref{tab:subt} whose premises are still in $\srel$. 
To this end, consider $U \subt[m_{U,V}] V$ in $\srel$ and split cases on the last rule used to derive it. 

\proofrule{f-end}
We have $U = V = \End$, hence the thesis is immediate by \refrule{f-end}. 

\proofrule{f-tag-in}
We have $U = \Tags\role\In\Tag_i.U_i$ and $V = \JTags\role\In\Tag_j.V_j$ with $I\subseteq J$ and 
$U_i\subt[k_i]V_i$ with $k_i\le m_{U,V}$, for all $i \in I$. 
By definition we have $m_{U_i,V_i}\le k_i \le m_{U,V}$ and 
$\ple{U_i,V_i}\in \Sk(U,V)\subseteq\Sk(S,T)$, for all $i \in I$, 
hence we conclude by rule \refrule{f-tag-in}. 

\proofrule{f-tag-out-1}
Analogous to the previous case.

\proofrule{f-tag-out-2}
We have $U = \Tags[i\in I\cup J]\role\Out\Tag_i.U_i$ and $V = \Tags\role\Out\Tag_i.V_i$ and 
$U_i\subt[k_i]V_i$, for all $i \in I$, and $k_j < m_{U,V}$, for some $j \in I$. 
By definition we have $m_{U_j,V_j}\le k_j < m_{U,V}$ and 
$\ple{U_i,V_i}\in \Sk(U,V)\subseteq\Sk(S,T)$, for all $i \in I$, 
hence we conclude by rule \refrule{f-tag-out-2}. 
\end{proof}

\begin{lemma}
  \label{lem:bounded_derivation}
  Let $S \subt[n]^m T$ if and only if $S \subt[n] T$ is the
  conclusion of a derivation in which every rank annotation is at
  most $m$. Then $S \subt[n] T$ if and only $S \subt[n]^m T$ for
  some $m$.
\end{lemma}
\begin{proof}
  The ``if'' part is obvious. Concerning the ``only if'' part, by
  \cref{lem:regular_derivation} we deduce that there exists a
  regular proof tree whose conclusion is $S \subt[n] T$. Since this
  tree is regular and has at least one judgment (in its root), the
  set of rank annotations occurring in it is finite and non
  empty. Let $m$ be the maximum annotation in this tree. We conclude
  $S \subt[n]^m T$.
\end{proof}

\begin{theorem}
  $\subt$ is a preorder.
\end{theorem}
\begin{proof}
  The proof that $\subt$ is reflexive is trivial, since
  $S \subt[n] S$ is derivable for every $n$. Concerning
  transitivity, by \cref{lem:bounded_derivation} it suffices to show
  that each judgment in the set
  \[
    \srel \eqdef \set{
      S \subt[n_1 + (1 + m)n_2] T \mid S \subt[n_1]^m U \wedge U \subt[n_2] T
    }
  \]
  is derivable using the rules in \cref{tab:subt} from premises that
  are also in $\srel$.
  %
  Suppose $S \subt[n] T \in \srel$. Then there exist $U$, $n_1$, $m$
  and $n_2$ such that $S \subt[n_1]^m U$ and $U \subt[n_2] T$ and
  $n = n_1 + (1 + m)n_2$.
  %
  We reason by cases on the last rules applied to derive
  $S \subt[n_1] U$ and $U \subt[n_2] T$.

  \proofrule{f-end}
  %
  Then $S = U = T = \End$ hence $S \subt[n] T$ is derivable by \refrule{f-end}.

  \proofrule{f-tag-in}
  %
  Then $S = \Tags\role\In\Tag_i.S_i$ and $U = \Tags[i\in J]\role\In\Tag_i.U_i$
  and $T = \Tags[i\in K]\role\In\Tag_i.T_i$ and $I \subseteq J \subseteq K$ and
  $S_i \subt[n_{1i}]^m U_i$ and $n_{1i} \leq n_1$ for every $i\in I$ and $U_i
  \subt[n_{2i}] T_i$ and $n_{2i} \leq n_2$ for every $i\in J$.
  %
  By definition of $\srel$ we have that $S_i \subt[n_{1i} + (1 + m)n_{2i}] T_i
  \in \srel$ for every $i\in I$.
  %
  Observe that $n_{1i} + (1 + m)n_{2i} \leq n_1 + (1 + m)n_2 = n$ for every
  $i\in I$ hence $S \subt[n] T$ is derivable by \refrule{f-tag-in}.

  \proofrule{f-tag-out-1}
  %
  Then $S = \Tags\role\Out\Tag_i.S_i$ and
  $U = \Tags\role\Out\Tag_i.U_i$ and $T = \Tags\role\Out\Tag_i.T_i$
  and $S_i \subt[n_{1i}]^m U_i$ and $n_{1i} \leq n_1$ and
  $U_i \subt[n_{2i}] T_i$ and $n_{2i} \leq n_2$ for every $i\in I$.
  %
  By definition of $\srel$ we have that
  $S_i \subt[n_{1i} + (1 + m)n_{2i}] T_i \in \srel$ for every
  $i\in I$.
  %
  Observe that $n_{1i} + (1 + m)n_{2i} \leq n_1 + (1 + m)n_2 = n$
  for every $i\in I$ hence $S \subt[n] T$ is derivable by
  \refrule{f-tag-out-1}.

  \proofcase{Case \refrule{f-tag-out-1} and \refrule{f-tag-out-2}}
  %
  Then $S = \Tags\role\Out\Tag_i.S_i$ and
  $U = \Tags\role\Out\Tag_i.U_i$ and
  $T = \Tags[i\in J]\role\Out\Tag_i.T_i$ and $J \subseteq I$ and
  $S_i \subt[n_{1i}]^m U_i$ and $n_{1i} \leq n_1$ for every $i\in I$
  and $U_i \subt[n_{2i}] T_i$ for every $i\in J$ and $n_{2k} < n_2$
  for some $k\in J$.
  %
  By definition of $\srel$ we have that
  $S_i \subt[n_{1i} + (1 + m)n_{2i}] T_i \in \srel$ for every
  $i\in J$.
  %
  Observe that $n_{1k} + (1 + m)n_{2k} < n_1 + (1 + m)n_2 = n$ hence
  $S \subt[n] T$ is derivable by \refrule{f-tag-out-2}.

  \proofcase{Case \refrule{f-tag-out-2} and \refrule{f-tag-out-1}}
  %
  Then $S = \Tags\role\Out\Tag_i.S_i$ and
  $U = \Tags[i\in J]\role\Out\Tag_i.U_i$ and
  $T = \Tags[i\in J]\role\Out\Tag_i.T_i$ and $J \subseteq I$ and
  $S_i \subt[n_{1i}]^m U_i$ for every $i\in J$ and $n_{1k} < n_1$
  for some $k\in J$ and $U_i \subt[n_{2i}] T_i$ for every $i\in J$
  and $n_{2i} \leq n_2$ for every $i\in J$.
  %
  By definition of $\srel$ we have that
  $S_i \subt[n_{1i} + (1 + m)n_{2i}] T_i \in \srel$ for every
  $i\in J$.
  %
  Observe that $n_{1k} + (1 + m)n_{2k} < n_1 + (1 + m)n_2 = n$ hence
  $S \subt[n] T$ is derivable by \refrule{f-tag-out-2}.

  \proofrule{f-tag-out-2}
  %
  Then $S = \Tags\role\Out\Tag_i.S_i$ and
  $U = \Tags[i\in J]\role\Out\Tag_i.U_i$ and
  $T = \Tags[i\in K]\role\Out\Tag_i.T_i$ and
  $K \subseteq J \subseteq I$ and $S_i \subt[n_{1i}]^m U_i$ for
  every $i\in J$ and $n_{1j} < n_1$ for some $j\in J$ and
  $U_i \subt[n_{2i}] T_i$ for every $i\in K$ and $n_{2k} < n_2$ for
  some $k\in K$.
  %
  By definition of $\srel$ we have that
  $S_i \subt[n_{1i} + (1 + m)n_{2i}] T_i \in \srel$ for every
  $i\in K$.
  %
  Observe that
  \[
    \begin{array}{rcll}
      n_{1k} + (1 + m)n_{2k} & \leq & m + (1 + m)n_{2k} & \text{since $n_{1k} \leq m$}
      \\
      & < & 1 + m + (1 + m)n_{2k}
      \\
      & = & (1 + m)(1 + n_{2k})
      \\
      & \leq & (1 + m)n_2 & \text{since $n_{2k} < n_2$}
      \\
      & < & n_1 + (1 + m)n_2 & \text{since $n_{1j} < n_1$}
    \end{array}
  \]
  hence $S \subt[n] T$ is derivable by \refrule{f-tag-out-2}.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

